Power-to-X in Energy Hubs: Operations and Policies Supporting the Scale-Up of Renewable Fuel Production

Power-to-X (P2X) needs to scale up rapidly to provide the fuels required in the hard-to-decarbonize industrial and heavy transport sector. Only recently, the European Commission proposed requirements for \textit{renewable} fuels. P2X energy hubs enable efficient synergies between energy infrastructures, production facilities, and storage options. In this study, we explore the optimal operation of an energy hub by leveraging the flexibility of P2X including hydrogen, methanol, and ammonia synthesizers, and analyze potential revenue streams such as the day-ahead and ancillary service markets. We propose EnerHub2X, a mixed-integer linear program that maximizes the hub's profit based on current market prices, considering technical constraints of P2X such as unit commitment and non-linear efficiencies. We model a representative Danish energy hub and find that without price incentives, it mainly produces liquid hydrogen and sells renewable electricity. Only by adding a price premium of about 50\% (0.16 \euro{}/kg) to the conventional fuel prices, sufficient amounts of renewable ammonia and methanol are produced. To utilize production efficiently, on-site renewable capacity and P2X must be carefully aligned. We show that renewable power purchase agreements can provide flexibility while complying with the rules set by the European Commission.

==> Mathematical Model Source/EnergyHub2X.tex <==
\begin{equation}
\begin{aligned}
& \underset{\Xi^{\mathrm{MIP}}
}{\operatorname{Maximize}}  
 \sum_{(a,e) \in SE, t} C^{export}_{a,e,t} Q^{sale}_{a,e,t} - \sum_{(a,e) \in BE, t} C^{import}_{a,e,t} Q^{buy}_{a,e,t}  
- \sum_{g,t}F^{total}_{g,t} C^{O\&M}_{g}  - \sum_{g,t} C^{SC}_{g,t}  \\
& \hspace{1cm}+ \sum_{(a,e) \in (SE \cap E^V), g \in T^{v}, t} Q^{rene}_{a,g,e,t}  C^{export}_{a,e,t} \\
&\text {\textbf{Subject to} (\ref{eq:FuelUse}) - (\ref{eq: Demand should be equal to D})}
\label{eq: ObjectivefunctionderPro}
\end{aligned}
\end{equation}
\begin{equation}
    F^{fuel}_{g,e,t}  =  F^{total}_{g,t} EF^{import}_{g,e,t}  \quad \forall g,\forall e,\forall t
    \label{eq:FuelUse}
\end{equation}
\begin{equation}
    G^{fuel}_{g,e,t} = F^{total}_{g,t} EF^{export}_{g,e,t} EF^{total}_{g,t}  \quad \forall g \in (EF^{NG} \cap G^{P}) ,\forall e,\forall t
    \label{eq:Generation}
\end{equation}
\begin{equation}
     F^{total}_{g,t} =  P^{max}_{g} \sum_{k \in K} P^{load}_{g,t,k} \hat{U}_{g,k}  \quad \forall g \in EF^{G} ,\forall e,\forall t
    \label{eq:ImportFuelCurve}
\end{equation}
\begin{equation}
     G^{fuel}_{g,e,t} =  P^{max}_{g} EF^{export}_{g,e,t} \sum_{k \in K} P^{load}_{g,t,k}  \hat{U}_{g,k} \hat{EF}^{total}_{g,k} \quad \forall g \in EF^{G}  ,\forall e,\forall t 
    \label{eq:ProductionFuelCurve}
\end{equation}
\begin{equation}
     \sum_{k \in K}  P^{load}_{g,t,k} =  O^{online}_{g,t} \quad \forall g \in EF^{G} , \forall t
    \label{eq:Weights}
\end{equation}
\begin{equation}
     P^{load}_{g,t,k} + P^{load}_{g,t,k-1} \geq  0 \quad \forall g \in EF^{G}, \forall t, \forall k
    \label{eq:LinkWeights}
\end{equation}
\begin{equation}
       \sum_{e \in E} \left [G^{fuel}_{g,e,t} - G^{fuel}_{g,e,t-1} \right] \leq R^{up}_{g}  \quad \forall g \in (G^{NUC} \cap G^{R}) , \forall t
\label{eq:Ramp up no UC}
\end{equation}
\begin{equation}
       \sum_{e \in E} \left [G^{fuel}_{g,e,t-1} - G^{fuel}_{g,e,t} \right] \leq R^{down}_{g}  \quad \forall g \in (G^{NUC} \cap G^{R}), \forall t
\label{eq:Ramp Down no UC}
\end{equation}
\begin{equation}
       \sum_{e \in E} \left [G^{fuel}_{g,e,t} - G^{fuel}_{g,e,t-1} \right] \leq R^{up}_{g} O^{online}_{g,t-1} + P^{min}_{g} (1-O^{online}_{g,t-1})  \quad \forall g \in (G^{UC} \cap G^{R}), \forall t
\label{eq:Ramp Up UC}
\end{equation}
\begin{equation}
       \sum_{e \in E} \left [G^{fuel}_{g,e,t-1} - G^{fuel}_{g,e,t} \right] \leq R^{down}_{g} O^{online}_{g,t} + P^{min}_{g} (1-O^{online}_{g,t})  \quad \forall g \in (G^{UC} \cap G^{R}), \forall t
\label{eq:Ramp Down UC}
\end{equation}
\begin{equation}
       F^{total}_{g,t}      \leq  P^{max}_{g}O^{online}_{g,t}  \quad \forall g \in G^{UC}, \forall t 
\label{eq:max production}
\end{equation}
\begin{equation}
       F^{total}_{g,t}      \geq  P^{min}_{g}O^{online}_{g,t}  \quad \forall g \in G^{UC}, \forall t 
\label{eq:minproduction}
\end{equation}
\begin{equation}
       C^{SC}_{g,t} = C^{StartCost}_{g} \left( O^{online}_{g,t} - O^{online}_{g,t-1} \right)   \quad \forall g \in G^{UC}, \forall t 
\label{eq:Startupcost}
\end{equation}
\begin{equation}
       F^{total}_{g,t} \leq P^{max}_{g} P^{profile}_{g,t}  \quad \forall g, \forall t 
\label{eq:limitFuelusetot}
\end{equation}
\begin{equation}
       G^{fuel}_{g,e,t} \leq P^{max}_{g} P^{profile}_{g,t} EF^{total}_{g} EF^{export}_{g,e} \quad \forall g, \forall t 
\label{eq:LimitGeneration}
\end{equation}
\begin{equation}
      \sum_{g \in G} F^{fuel}_{g,e,t} \leq F^{max}_{g,e} \quad \forall e, \forall t 
\label{eq:LimitFuelUse}
\end{equation}
\begin{equation}
    Q^{buy}_{(a,e) \in BE,t} + \sum_{a \in FL^{in}} F^{flow}_{a,n,e,t} + \sum_{g \in (LT \cap OF)} G^{fuel}_{g,e,t} =   Q^{sale}_{(a,e) \in SE,t}  + \sum_{a \in FL^{out}} F^{flow}_{a,n,e,t} + \sum_{g \in (LT \cap IF)} F^{fuel}_{g,e,t}          \quad \forall a,\forall n, \forall e, \forall t
    \label{eq:EnergyBalance}
\end{equation}
\begin{equation}
Q^{sale}_{a,e,t} + D^{slack}_{a,e,t,d \in D^I} - D^{slack}_{a,e,t,d \in D^E} = D_{a,e,t} \quad \forall a, \forall e \in E^{D}, \forall t
\label{eq:Demand Balance}
\end{equation}
\begin{equation}
    V^{storage}_{g,t} = V^{storage}_{g,t-1} + F^{total}_{g,t} - \sum_{e \in E}  G^{fuel}_{g,e,t} EF^{export}_{g,e,t}    \quad \forall g \in G^{s} ,\forall e,\forall t \in T/t=1
    \label{eq:ProductionStorage}
\end{equation}
\begin{equation}
    V^{storage}_{g,t} \leq Vol^{max}_{g}    \quad \forall g \in G^{s},\forall t
    \label{eq:max volume}
\end{equation}
\begin{equation}
    V^{storage}_{g,t=1} = V^{storage}_{g,t=N}   \quad \forall g \in G^{s} 
    \label{eq:volinitLast}
\end{equation}
\begin{equation}
    V^{storage}_{g,t} = Vol^{init}   \quad \forall g \in G^{s} ,\forall t=1
    \label{eq:Volinit}
\end{equation}
\begin{equation}
Q^{Rene}_{a,g,e,t} = P^{max}_{g} P^{profile}_{g,t} EF^{export}_{g,e,t} - G^{fuel}_{g,t,e}   \quad \forall a \in SE, \forall g \in T^{V}, \forall e, \forall t 
\label{eq:Renewable Balance}
\end{equation}
\begin{equation}
Q^{Rene}_{a,g,e,t} \leq P^{max}_{g} P^{profile}_{g,t} EF^{export}_{g,e,t}    \quad \forall a \in SE, \forall g \in T^{V}, \forall e, \forall t
\label{eq:Renewable limit}
\end{equation}
\begin{equation}
     D^{Response}_{a,e,t} \geq (1 - \eta) D_{a,e,t}  \quad \forall a, \forall e \in E^{D}, \forall t
    \label{eq: DemandRespone can be less than D}
\end{equation}
\begin{equation}
     D^{Response}_{a,e,t} \leq (1 + \eta) D_{a,e,t}  \quad \forall a, \forall e \in E^{D}, \forall t
    \label{eq: DemandResponse more than D}
\end{equation}
\begin{equation}
    \sum_{t \in T} D^{Response}_{a,e,t} = \sum_{t \in T} D_{a,e,t}  \quad \forall a, \forall e \in E^{D}, 
    \label{eq: DemandResponse should be equal to D}
\end{equation}
\begin{equation}
    Q^{sale}_{a,e,t} \geq D^{Response}_{a,e,t}  \quad \forall a, \forall e \in E^{D}, \forall t
    \label{eq: Salemore than Demand}
\end{equation}
\begin{equation}
    \sum_{t \in T} D^{Response}_{a,e,t} = \sum_{t \in T} Q^{sale}_{a,e,t}  \quad \forall a, \forall e \in E^{D}, 
    \label{eq: Demand should be equal to D}
\end{equation}


==> Mathematical Model Source/Nomeclature.tex <==
%start nomenclature
%Indices
\nomenclature[A]{\(g\)}{Available technologies/Process}
\nomenclature[A]{\(e\)}{Energy carriers/Fuels}
\nomenclature[A]{\(t\)}{Dispatching periods}
\nomenclature[A]{\(a\)}{Areas}
\nomenclature[A]{\(d\)}{Direction of flows, \{input/output\}}

%Sets
\nomenclature[B]{\(\mathbb{G}\)}{Set of dispatchable technology units}

\nomenclature[B]{\(\mathbb{G}^{R}\)}{Subset of dispatchable  technology units with Ramping technical constraint}

\nomenclature[B]{\(\mathbb{G}^{S}\)}{Subset of storage technology units}

\nomenclature[B]{\(\mathbb{G}^{UC}\)}{Subset of dispatchable technology units with unit commitment constraints (on/off)}

\nomenclature[B]{\(\mathbb{G}^{LD}\)}{Subset of dispatchable  technology units with efficiency varying based on load dependency}

\nomenclature[B]{\(\mathbb{G}^{AS^{+}}\)}{Subset of dispatchable  technology units able to provide Up regulation ancillary services}

\nomenclature[B]{\(\mathbb{G}^{AS^{-}}\)}{Subset of dispatchable  technology units able to provide Down regulationancillary services}


\nomenclature[B]{\(\mathbb{G}^{Var}\)}{Subset of variable energy technology units}

\nomenclature[B]{\(\mathbb{G}_{a}\)}{Mapping set of technologies to areas}

\nomenclature[B]{\(\mathbb{E}\)}{Set of fuels}

\nomenclature[B]{\(\mathbb{E}^{In}_{g}\)}{Mapping set of feedstock fuels to corresponding technologies}

\nomenclature[B]{\(\mathbb{E}^{Out}_{g}\)}{Mapping set of produced fuels from technologies}

\nomenclature[B]{\(\mathbb{E}^{Buy}_{a}\)}{Mapping set of feedstock fuels purchased from areas}

\nomenclature[B]{\(\mathbb{E}^{Sell}_{a}\)}{Mapping set of end product fuels sold to area}

\nomenclature[B]{\(\mathbb{E}^{D}\)}{Subset of fuels associated with demand constraint}

\nomenclature[B]{\(\mathbb{E}^{Var}\)}{Subset of fuels characterized by variable production}

\nomenclature[B]{\(\mathbb{E}^{Def}_{g}\)}{Mapping set of fuels defining the technical characteristics of technology}

\nomenclature[B]{\(\mathbb{F}_{(a,a)}\)}{Mapping set of fuels flow from area to area}

%\nomenclature[B]{\(\mathbb{F}^{+}_{a}\)}{Mapping set of energy carriers input flow to area.}
%\nomenclature[B]{\(\mathbb{F}^{-}_{a}\)}{Mapping set of energy carriers leaving flow from area.}
\nomenclature[B]{\(\mathbb{K}\)}{Piecewise linear approximation brakepoints of the load dependent production efficiency curve}

%Parameters definition
\nomenclature[C]{\(\sigma^{in}_{g,e}\)}{Percentage of fuel $e $ used as a feedstock in technology $g$}

\nomenclature[C]{\(\sigma^{out}_{g,e}\)}{Percentage of fuel $e $ produced by technology $g$}

\nomenclature[C]{\(F^{out}_{g,e}\)}{Fixed amount of fuel $e$ produced by technology $g$}

\nomenclature[C]{\(F^{in}_{g,e}\)}{Fixed amount of fuel $e $ used as a feedstock in technology $g$}

\nomenclature[C]{\(\Theta_{g}\)}{Percentage of activity state change from consumption to production of technology $g$}

\nomenclature[C]{\(U_{g,k}\)}{Load levels of technology $g$ at break point $k$}

\nomenclature[C]{\(\Theta_{g,k}\)}{Percentage of activity state change from consumption to production of technology $g$ in breakpoint $k$}

\nomenclature[C]{\(P^{max}_{g}\)}{Maximum production level/capacity of technology $g$}

\nomenclature[C]{\(R^{+}_{g}/R^{-}_{g}\)}{Maximum up/down reserve capacity of technology $g$}

%\nomenclature[C]{\(R^{-}_{g}\)}{Maximum down reserve capacity of %technology $g \in \mathbb{G}$}

\nomenclature[C]{\(P^{min}_{g}\)}{Minimum production level of technology $g$}

\nomenclature[C]{\(SOC^{max}_{g}\)}{Maximum volume of storage technology $g$}

\nomenclature[C]{\(SOC^{init}_{g}\)}{Initial volume of storage technology $g$ for $t=1$}

\nomenclature[C]{\(R^{up}_{g}/R^{down}_{g}\)}{Ramp up/down rate limit of technology $g$}

%\nomenclature[C]{\(R^{Down}_{g}\)}{Ramp down rate limit of technology $g %\in \mathbb{G}$}

\nomenclature[C]{\(C^{var}_{g}\)}{Variable operating cost of $g $}

\nomenclature[C]{\(C^{start}_{g}\)}{Start-up cost of dispatchable technology $g$}

%nomenclature[C]{\(Cf_{g,t}\)}{Capacity factor of technology $g %\in \mathbb{G}$ in period $t$}

\nomenclature[C]{\(\pi^{buy}_{a,e,t}\)}{Price of feedstock fuel $e$ bought from area $a$ in period $t$}

\nomenclature[C]{\(\pi^{sell}_{a,e,t}\)}{Price of end product fuel $e$ sold at area $a$ in period $t$}

\nomenclature[C]{\(D_{a,e,t}\)}{Demand at area $a$  of end product fuel $e$ in period $t$}

\nomenclature[C]{\(X^{cap}_{a,e,t}\)}{Maximum flow of fuel $e$ from area $a$ in period $t$}

\nomenclature[C]{\(\pi^{activation}_{t}\)}{Price for reserve activation in period $t$}

\nomenclature[C]{\(\pi^{+}_{t}/\pi^{-}_{t}\)}{mFRR Up/Down regulation reserve capacity payment in period $t$}

%\nomenclature[C]{\(\pi^{-}_{t}\)}{mFRR Down regulation reserve capacity %payment in period $t \in \mathbb{T}$}

\nomenclature[C]{\(\pi^{\omega}_{t}\)}{Activation probability in period $t$}

\nomenclature[C]{\(P^{profile}_{g,t}\)}{Capacity factor of technology $g$ in period $t$}

%-----------------------------------------------------------------
%Variables definition
\nomenclature[D]{\(x^{in}_{g,e,t}\)}{Amount of feedstock fuel $e $ consumed in technology $g$ in period $t$}

\nomenclature[D]{\(x^{out}_{g,e,t}\)}{Amount of produced fuel $e $ from technology $g $ in period $t$}

\nomenclature[D]{\(x^{total}_{g,t}\)}{Level of activity of technology $g$ in period $t$}

\nomenclature[D]{\(soc_{g,t}\)}{State of charge for technology $g$ in period $t$}

\nomenclature[D]{\(f^{flow}_{a,a',e,t}\)}{Flow from area $a$ to $a'$ of fuel $e$ in period $t$}

\nomenclature[D]{\(q^{buy}_{a,e,t}\)}{Quantity of feedstock fuel $e \in \mathbb{E}^{buy}_{a}$ bought from area $a$ in period $t$}

\nomenclature[D]{\(q^{sell}_{a,e,t}\)}{Quantity of end product fuel $e \in \mathbb{E}^{sell}_{a}$ sold to area $a$ in period $t$}

\nomenclature[D]{\(c^{start}_{g,t}\)}{Start up cost of technology $g$ in period $t$}

\nomenclature[D]{\(o_{g,t}\)}{Binary indicating online/offline status of technology $g$ in period $t$}
\nomenclature[D]{\(u_{g,t}\)}{Binary indicating when status up occurs of technology $g$ in period $t$}

\nomenclature[D]{\(w^{sos2}_{g,t,k}\)}{Activity level of technology $g$ in period $t$ at break point $k$}

\nomenclature[D]{\(\nu_{g,t}\)}{Binary indicating charging or discharging status of storage technology $g$ in period $t$}

%Write the extra variables due to reserve
%Up regulation
\nomenclature[D]{\(x^{in^{+}}_{g,e,t}/x^{in^{-}}_{g,e,t}\)}{Amount of feedstock fuel $e$ consumed in technology $g$ in period $t$ for activation of Up/Down regulation service}

\nomenclature[D]{\(x^{out^{+}}_{g,e,t}/x^{out^{-}}_{g,e,t}\)}{Amount of produced fuel $e$ from technology $g$ in period $t$  for activation of Up/Down-regulation service}

\nomenclature[D]{\(x^{total^{+}}_{g,t}/x^{total^{-}}_{g,t}\)}{Level of activity of technology $g$ in period $t$  for activation of Up/Down-regulation service}

\nomenclature[D]{\(x^{cap^{+}}_{g,t}/x^{cap^{-}}_{g,t}\)}{Capacity reserved $g $ in period $t$ for providing Up/Down-regulation service}

\nomenclature[D]{\(q^{{buy}^{+}}_{a,e,t}/q^{{buy}^{-}}_{a,e,t}\)}{Quantity of feedstock fuel $e \in \mathbb{E}^{buy}_{a} $ bought from area $a$ in period $t$ for energy hub activation of Up/Down regulation service }

\nomenclature[D]{\(q^{{sell}^{+}}_{a,e,t}/q^{{sell}^{-}}_{a,e,t}\)}{Quantity of end product fuel $e \in \mathbb{E}^{sell}_{a}$ sold to area $a$ in period $t$ for energy hub activation of Up/Down regulation service}

\nomenclature[D]{\(f^{{flow}^{+}}_{a,a',e,t}/f^{{flow}^{-}}_{a,a',e,t}\)}{Flow from area $a$ to $a' $ of fuel $e$ in period $t$ for Up/Down regulation activity }

%Down
%\nomenclature[D]{\(x^{In^{-}}_{g,e,t}\)}{Amount of feedstock fuel $e \in %\mathbb{E}$ consumed in technology $g \in \mathbb{G}$ in period $t \in %\mathbb{T}$ for activation of Down regulation service}
%
%\nomenclature[D]{\(x^{Out^{-}}_{g,e,t}\)}{Amount of produced fuel $e \in %\mathbb{E}$ from technology $g \in \mathbb{G}$ in period $t \in %\mathbb{T}$  for activation of Down-regulation service}

%\nomenclature[D]{\(x^{total^{-}}_{g,t}\)}{Level of activity of technology %$g \in \mathbb{G}$ in period $t \in \mathbb{T}$  for activation of %Down-regulation service}

%\nomenclature[D]{\(x^{cap^{-}}_{g,t}\)}{Capacity reserved $g \in %\mathbb{G}$ in period $t \in \mathbb{T}$ for providing Down-regulation %service}

%\nomenclature[D]{\(f^{{Buy}^{-}}_{a,e,t}\)}{Quantity of feedstock fuel $e %\in \mathbb{E}$ bought from area $a \in \mathbb{A}$ in period $t \in %\mathbb{T}$ for energy hub activation of Down regulation service }
%
%\nomenclature[D]{\(f^{{Sell}^{-}}_{a,e,t}\)}{Quantity of end product fuel %$e \in \mathbb{E}$ sold to area $a \in \mathbb{A}$ in period $t \in %\mathbb{T}$ for energy hub activation of Down regulation service}
%
%\nomenclature[D]{\(f^{{flow}^{-}}_{a,a',e,t}\)}{Flow from area $a \in %\mathbb{A}$ to $a' \in \mathbb{A}$ of fuel $e \in \mathbb{E}$ in period $t %\in \mathbb{T}$ for Down regulation activity }

\nomenclature[D]{\(\lambda_{g,t}\)}{Binary indicating activity for providing Up or Down ancillary services of technology $g $ in period $t$}



==> MissingFunctions.tex <==
%add this on elsarticle harv 
%At line 950 before doi

%  print.url output
